Dex-Net 3.0: Computing Robust Robot Vacuum Suction Grasp Targets in Point Clouds using a New Analytic Model and Deep Learning

Vacuum-based end effectors are widely used in industry and are often preferred over parallel-jaw and multifinger grippers due to their ability to lift objects with a single point of contact. Suction grasp planners often target planar surfaces on point clouds near the estimated centroid of an object. In this paper, we propose a compliant suction contact model that computes the quality of the seal between the suction cup and local target surface and a measure of the ability of the suction grasp to resist an external gravity wrench. To characterize grasps, we estimate robustness to perturbations in end-effector and object pose, material properties, and external wrenches. We analyze grasps across 1,500 3D object models to generate Dex-Net 3.0, a dataset of 2.8 million point clouds, suction grasps, and grasp robustness labels. We use Dex-Net 3.0 to train a Grasp Quality Convolutional Neural Network (GQ-CNN) to classify robust suction targets in point clouds containing a single object. We evaluate the resulting system in 350 physical trials on an ABB YuMi fitted with a pneumatic suction gripper. When evaluated on novel objects that we categorize as Basic (prismatic or cylindrical), Typical (more complex geometry), and Adversarial (with few available suction-grasp points) Dex-Net 3.0 achieves success rates of 98$\%$, 82$\%$, and 58$\%$ respectively, improving to 81$\%$ in the latter case when the training set includes only adversarial objects. Code, datasets, and supplemental material can be found at http://berkeleyautomation.github.io/dex-net .

==> graphical_model_details.tex <==
\section{Parameters of Graphical Model}
\label{graphical-details}

Our graphical model is illustrated in \figref{graphical-model} and models $p(S, \bg, \bx, \by)$ as the product of a state distribution $p(\bx)$, an observation model $p(\by | \bx)$, a grasp candidate model $p(\bg | \bx)$, and a grasp success model $p(S | \bg, \bx)$.

We model the state distribution as $p(\bx) = p(\gamma) p(\mO) p(T_{o} | \mO)  p(T_{c})$.
We model $p(\gamma)$ as a Gaussian distribution $\mN(0.5, 0.001)$ truncated to $[0,1]$.
We model $p(\mO)$ as a discrete uniform distribution over 3D objects in a given dataset.
We model $p(T_{o} | \mO) = p(T_{o} | T_{s}) p(T_{s} | \mO) $, where is $p(T_{s} | \mO)$ is a discrete uniform distribution over object stable poses and $p(T_{o} | T_{s})$ is uniform distribution over 2D poses: $\mU([-0.1,0.1]\times[-0.1,0.1]\times[0,2\pi))$.
We compute stable poses using the quasi-static algorithm given by Goldberg et al.~\cite{goldberg1999part}.
We model $p(T_{c})$ as a uniform distribution on spherical coordinates $r, \theta, \phi \sim \mU([0.65, 0.75]\times[0,2\pi)\times[0.05\pi, 0.1\pi])$, where the camera optical axis always intersects the center of the table.

Our distribution over grasps is a uniform distribution over pairs of antipodal points on the object surface that are parallel to the table plane.
We sample from this distribution for a fixed coefficient of friction $\mu = 0.6$ and reject samples outside the friction cone or non-parallel to the surface.

We model images as $\by = \alpha * \hat{\by} + \epsilon$ where $\hat{\by}$ is a rendered depth image created using OSMesa offscreen rendering.
We model $\alpha$ as a Gamma random variable with shape$=1000.0$ and scale=$0.001$.
We model $\epsilon$ as Gaussian Process noise drawn with measurement noise $\sigma=0.005$ and kernel bandwidth $\ell = \sqrt{2}px$.

We compute grasp robustness metrics using the graphical model and noise parameters of~\cite{seitalarge}.

